PWTO: A Heuristic Approach for Trajectory Optimization in Complex Terrains

This paper considers a trajectory planning problem for a robot navigating complex terrains, which arises in applications ranging from autonomous mining vehicles to planetary rovers. The problem seeks to find a low-cost dynamically feasible trajectory for the robot. The problem is challenging as it requires solving a non-linear optimization problem that often has many local minima due to the complex terrain. To address the challenge, we propose a method called Pareto-optimal Warm-started Trajectory Optimization (PWTO) that attempts to combine the benefits of graph search and trajectory optimization, two very different approaches to planning. PWTO first creates a state lattice using simplified dynamics of the robot and leverages a multi-objective graph search method to obtain a set of paths. Each of the paths is then used to warm-start a local trajectory optimization process, so that different local minima are explored to find a globally low-cost solution. In our tests, the solution cost computed by PWTO is often less than half of the costs computed by the baselines. In addition, we verify the trajectories generated by PWTO in Gazebo simulation in complex terrains with both wheeled and quadruped robots. The code of this paper is open sourced and can be found at https://github.com/rap-lab-org/public_pwto.

==> sections/intro-OLD.tex <==

This work considers a trajectory planning problem for a dynamic wheeled robot in complex terrains.
The terrain is represented as a static 2D continuous potential field that characterizes the traversal cost of the robot at each location~\cite{chavez2018learning,papadakis2013terrain}, and the goal of the problem is to find a dynamically feasible low-cost trajectory for the robot (Fig.~\ref{pwdc:fig:fig1}).
This problem arises in many applications ranging from planetary rovers~\cite{strader2020perception}, exploration~\cite{Fan-RSS-21} to autonomous mining.
% Consider an autonomous vehicle with non-holonomic constraints and acceleration limits navigating in a mine.
The problem is challenging as it requires solving a non-linear optimization problem to find a (globally) low-cost trajectory in complex terrains while ensuring (local) dynamically feasibility along the entire trajectory.

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/fig1.png}
	\caption{
% 		The goal of this work is to find a dynamically feasible, low-cost trajectory in a complex terrain.
		Oblique view of a complex non-flat terrain with a top-down view denoting a purple trajectory from start to goal for the robot identified in the lower right panel.
	}
	\label{pwdc:fig:fig1}
\end{figure}

In the literature, similar problems~\cite{natarajan2021interleaving,hoenig2022db} have been addressed with various methods, which are reviewed in the Related Work section.
Of close relevance to this work is a popular approach~\cite{andreasson2015fast,Fan-RSS-21} that first leverages a search-based method to solve a relaxed problem (e.g. by simplifying the  dynamics of the robot) to find a path or trajectory (i.e., an initial guess) that is globally near-optimal with respect to some discretization.
Then, the initial guess warm-starts a local trajectory optimization process to smooth the trajectory, enforce the constraints, and further reduce the cost.
This type of approach has two major limitations for the problem considered in this work.
First, it can lead to a highly sub-optimal solution that converges to a local minimum.
Second, the local trajectory optimization may require many iterations to converge due to the complicated objective function and the dynamic constraints of the robot.

To bypass these two limitations, we propose a heuristic method called Pareto-optimal Warm-started Trajectory Optimization (PWTO) with the following two key ideas.
First, PWTO relaxes the original (single-objective) trajectory optimization problem by ignoring the dynamics of the robot and formulating a graph-based multi-objective path planning (MOPP) problem, where each objective emphasizes a different aspect of the original trajectory optimization problem.
PWTO then solves this MOPP to obtain distinct Pareto-optimal paths\footnote{A solution path is Pareto-optimal if there exists no other solution that will yield an improvement in one objective without causing a deterioration in at least one of the other objectives.}, which are then used as the initial guesses to warm-start multiple local trajectory optimization processes.
By doing so, PWTO is able to explore different local minima and thus has a higher chance to find a low-cost solution.
Second, to avoid being trapped in an optimization process that take many iterations to converge, PWTO runs these processes in a round-robin fashion (i.e., alternate between these processes), and is thus able to report the converged solution in an anytime fashion.\footnote{The notion of ``anytime'' in PWTO is that, the first converged solution is quickly reported and other converged solutions are reported during the computation if they are cheaper. It differs from the anytime methods that iteratively improve the quality of the solution until the time budget depletes.}
As a result, the proposed PWTO method is able to obtain dynamically feasible low-cost trajectories in complex terrains (Fig.~\ref{pwdc:fig:fig1}).

We evaluate PWTO against baseline methods in various terrains.
The results show that PWTO can compute solutions with less than half of the cost of the baselines and is able to avoid being trapped in a specific optimization process.
We also run Gazebo simulation to verify the feasibility of the planned trajectory in several different terrains.

%The rest of this article is organized as follows.
%Sec.~\ref{pwdc:sec:related} reviews related work and Sec.~\ref{pwdc:sec:problem} formulates the problem.
%We then present PWTO in Sec.~\ref{pwdc:sec:method} with numerical results in Sec.~\ref{pwdc:sec:result}. We conclude and point out future work in Sec.~\ref{pwdc:sec:conclude}.





% address dynamics during the search can be computationally expensive: as it requires either generating dynamic feasible partial paths/motion primitives during the graph search, or spending a lot of time to pre-compute (in an offline manner) a large set of high quality motion primitives~\cite{}. 



%%% OLD
% Sampling-based method can quickly return a dynamic-feasible trajectory and keep refining the solution quality thereafter. However, the solution obtained are often far away from the optimum and the refinement converges slowly without domain-specific fine tuning.
% Search-based methods often provide high-quality solutions with global theoretic guarantees by using a set of pre-computed dynamic-feasible motion primitives.
% However, to ensure the dynamic-feasibility, a high-dimensional search space that captures the full state of the robot is often required, and search-based methods are in general hard to scale to high-dimensional search space due to the so-called curse of dimensionality.
% % However, the solution quality guarantee is often with respect to the graph
% In contrast, optimization-based methods scale well in high-dimensional state space by iteratively running local optimization but often rely on good initial guesses to warm-start the optimization in order to bypass local minima, which is common in cluttered environment.

% this work proposes a meta-heuristic method called Pareto-optimal Warm-start Direct Collocation (PWDC) that attempts to combine the benefits from both search-based and optimization-based methods to achieve the goals (i), (ii) and (iii) simultaneously.
% PWDC consists of two parts: the first part relaxes the dynamics and decompose the optimization objective function into multiple related criteria to formulate a multi-objective graph search problem. This graph search problem is then solved by explicitly optimizing the multiple criteria simultaneously and leads to a set of (globally) ``Pareto-optimal'' solution paths in the graph.\footnote{In multi-objective optimization, in general, there does not exist a single solution that can simultaneously optimize all the objectives at the same time. Thus one seek to find a set of Pareto-optimal solutions. A solution is Pareto-optimal is one cannot optimize one objectives without deteriorating another objective.}
% The second part uses the computed Pareto-optimal paths to warm-start multiple branches of (local) trajectory optimization. These branches are then optimized in an \emph{episodic} manner so that the entire computation will not get trapped in a branch that requires a lot of optimization iterations to converge.
% This episodic optimization enables PWDC to run in an \emph{anytime} fashion, as the first solution is often obtained quickly while better solutions can be possibly obtained as the computational time increases.

% The key ideas behind PWDC are: (i) decompose the single objective for trajectory optimization into multiple related criteria for global graph search in order to get distinct paths that emphasize on different aspects of the problem; (ii) warm-start the trajectory optimization using these distinct paths to bypass local minima; (iii) use an episodic optimization to plan trajectories in an \emph{anytime} fashion.
% To verify these ideas, we numerically evaluate PWDC against two baselines with several instances, and the solution cost computed by PWDC is less than half of the cost computed by the baselines.

